Improving Rare-Word Recognition of Whisper in Zero-Shot Settings

Whisper, despite being trained on 680K hours of web-scaled audio data, faces difficulty in recognising rare words like domain-specific terms, with a solution being contextual biasing through prompting. To improve upon this method, in this paper, we propose a supervised learning strategy to fine-tune Whisper for contextual biasing instruction. We demonstrate that by using only 670 hours of Common Voice English set for fine-tuning, our model generalises to 11 diverse open-source English datasets, achieving a 45.6% improvement in recognition of rare words and 60.8% improvement in recognition of words unseen during fine-tuning over the baseline method. Surprisingly, our model's contextual biasing ability generalises even to languages unseen during fine-tuning.

==> langauge_table.tex <==
\begin{table*}[t]
\vskip 0.15in
\small
\begin{center}
\begin{tabular}{l|ccc|ccc|ccc|cc}
\toprule
 &
\multicolumn{3}{c|}{Whisper} &
\multicolumn{3}{c|}{Whisper + Prompt} &
\multicolumn{3}{c|}{FancyName + Prompt} \\
\midrule
 Dataset & WER & R-WER & \CellWithForceBreak{OOV-\\WER}
 & WER & R-WER & \CellWithForceBreak{OOV-\\WER} & WER & R-WER & \CellWithForceBreak{OOV-\\WER} & R-WERR & \CellWithForceBreak{OOV-\\WERR} \\

\midrule
Common Voice & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 \\
Common Voice & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 \\
Common Voice & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 \\
Common Voice & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 \\
Common Voice & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 \\
Common Voice & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 \\
Common Voice & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 \\
Common Voice & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 \\
Common Voice & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 \\
Common Voice & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 \\
Common Voice & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 \\
Common Voice & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 \\
Common Voice & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 & 0.0 & 2.7 & 2.7 \\
\midrule
Average & 29.3 & \textbf{12.8} & \color{Highlight}55.2 \\

\bottomrule
\end{tabular}
\caption{\textbf{Detailed comparison of effective robustness across various datasets.} Although both models perform within 0.1\% of each other on LibriSpeech, a zero-shot Whisper model performs much better on other datasets than expected for its LibriSpeech performance and makes 55.2\% less errors on average. Results reported in word error rate (WER) for both models after applying our text normalizer.}
\label{robustness_table}
\end{center}
\vspace{-1em}
\end{table*}

